Discovering Invariant Rationales for Graph Neural Networks

Intrinsic interpretability of graph neural networks (GNNs) is to find a small subset of the input graph's features -- rationale -- which guides the model prediction. Unfortunately, the leading rationalization models often rely on data biases, especially shortcut features, to compose rationales and make predictions without probing the critical and causal patterns. Moreover, such data biases easily change outside the training distribution. As a result, these models suffer from a huge drop in interpretability and predictive performance on out-of-distribution data. In this work, we propose a new strategy of discovering invariant rationale (DIR) to construct intrinsically interpretable GNNs. It conducts interventions on the training distribution to create multiple interventional distributions. Then it approaches the causal rationales that are invariant across different distributions while filtering out the spurious patterns that are unstable. Experiments on both synthetic and real-world datasets validate the superiority of our DIR in terms of interpretability and generalization ability on graph classification over the leading baselines. Code and datasets are available at https://github.com/Wuyxin/DIR-GNN.

==> chapters/8_note.tex <==

Founded upon the causality independent mechanism \citep{pearl2000causality}, our strategy 


Specifically, our strategy consists of four modules: a rationale generator, an environment swapper, a feature encoder, and a predictor.
The rationale generator splits the input graph into causal and shortcut subgraphs, which are independent and dependent to environments, respectively.
The goal of environment swapper is to 



Our strategy reduces the importance of the environment-dependent shortcuts. It implicitly forces the GNN model to use the 




Aiming to approach rationales that capture the environment-invariant causal patterns, we formalize a new task of \underline{I}nvariant \underline{R}ationale \underline{D}iscovery (IRD) for intrinsically interpretable GNNs.
Briefly put, IRD distills the 



\emph{Invariant Rationale Discovery for GNNs} (IRD)



In this paper, we aim to approach the rationales, which not only latch on the causal patterns, but also generalize to OOD data.
Motivated by the insights of invariant learning \citep{IRM,REx,invariant-rationalization,Invariance}, we propose invariant rationale discovery (IRD)


We refer to this task as rationale discovery. Clearly, the main difficulty of rationale  


rationalization component,
representation learning,
predictor 


aiming to provide a recipe to train more 

causal features

=================================


A causal view of generalization formalizes this as identifying causal properties of the data-generating process behind the observed data. 


===========================================================

A critical outcome of this formalization is that such causal properties are provably impossible to recover solely from the joint distribution over inputs and outputs that a standard training set represents. In other words, spurious and reliable correlations cannot be distinguished from one another.

The causal formalization only serves to highlight that properties relevant to OOD generalization cannot be recovered from the joint distribution represented by a standard dataset, but can be informed by training across well-chosen environments.

Data points are usually collated into a single dataset, but this loses information. Our premise is that such environment elicit different 

The fact that observational data from multiple environments can be informative about causal properties of the data generating process may seem at odds with basic principles of causal reasoning. This is resolved when considering each environment as an intervention on the data generating process. Assuming these interventions only act on variables spuriously correlated with the output (hence the importance of a well-chosen partitioning), the causal mechanisms between non-intervened variables and the output will remain unchanged by the principle of independent causal mechanism. The statistical patterns inherent to the task thus remain stable across environments.

Here we ascribe the limits above to the ignorance of distribution shift and the failure of .
Motivated by insights of \citep{invariant-rationalization}, we 



they ignore the influence of distribution shift.

causal features, which hold the environment-invariant causal effect to the prediction

shortcut features, which 


rationale should identify causal features, while filter out shortcut patterns.


=====================================








=====================================


% TODO. 2. Narrow down to intrinsic interpretable models: (1) attention, (2) pooling categories.



% TODO. 3. Our key point: these explanations suffer from the environment invariance, struggle to figure out environment-invariant features (which reflect causal, stable, robust relations to prediction) & environment-dependent features (which suggest spurious, unstable, fragile relations to prediction); in turn, these invariant rationales endow models with better generalization ability & robustness. showing with a causal graph.

However, recent studies show that these models tend to exploit dataset biases as shortcuts to make predictions, rather than learn the semantic understanding and reasoning.
Here we focus on the background bias, where GNN models rely on spurious correlations between shortcut backgrounds and labels. This eventually results in their low generalizability on out-of-distribution samples and low adversarial robustness.

Previous empirical analysis indicates that the performance of GNN models could be mainly explained by the reliance of spurious statistical cues such as degree distribution, graph scales.

Current intrinsically explainable models can nevertheless lead to undesirable results in practice.
It is prone to highlighting spurious correlations between the input features and output as valid explanations.
While such correlations represent statistical relations present in the training data, and thus incorporated into the neural model, the impact of such features on the true outcome (as opposed to model's predictions) can change at test time.
In other words, these methods may select features that do not explain the underlying relationship between the inputs and outputs even though they may still be faithfully reporting the model's behavior.
We seek to modify the rationalization criterion to better tailor it to find causal features.

% TODO. 4. Our key idea: we introduce the invariant learning into the gnn models to discover the invariant rationales.

The implicit effect is to downweight the reliance on shortcut patterns, thereby discouraging the model from taking the shortcuts for prediction.

This helps ignoring spurious correlations and improves generalization but it requires explicit knowledge of desirable invariance. In comparison, our method discovers  invariance implicitly. We train a model to rely on input features that are similarly predictive (\ie invariant) across environments. The required expert knowledge is displaced to the specification of the partitioning into environments.


Our goal is to design a rationalization learning strategy that approximates finding causal rationale.
While assessing causality it challenging, we can approximate the task by searching subgraphs that are invariant. This notion was recently introduced in the context of invariant learning. The main idea is to highlight spurious (non-causal) variation by dividing the data into different environments. The same predictor, if based on causal features, should remain optimal in each environment separately.



% TODO. 5. Our main contributions.
In this paper, we propose invariant rationalization, a novel that incorporates the invariance into the intrinsic interpretability.
